Preprojective Analogue of the Cone Construction

We formulate a relative, representation theoretic, notion of the algebraic cone construction. This motivates a generalization of the cone corresponding to a preprojective algebra.

==> mypackagesnsf.tex <==
\usepackage{amsmath, amscd, amssymb, amsthm,amsfonts}
\usepackage{stmaryrd,euscript, mathrsfs, latexsym}
\usepackage{color}
\usepackage{hyperref} % links to refs
%\usepackage{diagrams}

\usepackage{lmodern}
\usepackage[T1]{fontenc} % things like \"o

\ifx\pdfoutput\undefined
\usepackage{graphicx}
\else
\fi

\ifx\xetex
\usepackage{fontspec}
\usefont{EU1}{lmr}{m}{n}%Latin Modern in OpenType format.
%\usefont{T1}{lmr}{m}{n}%Latin Modern in Type 1 format.
\else
\fi


% tikz diagrams
\usepackage{tikz}
\usetikzlibrary{matrix,arrows,positioning}
\tikzset{node distance=2cm, auto}

%datetime
%\usepackage[nodayofweek]{datetime}
\usepackage[UKenglish]{isodate}% http://ctan.org/pkg/isodate
\cleanlookdateon


% microtype fancy options

\usepackage[activate={true,nocompatibility},final,kerning=true,tracking=true,spacing=true,factor=1100,stretch=10,shrink=10]{microtype}
\SetTracking{encoding={*}, shape=sc}{0}

%\mathsurround=1pt
%\footskip=4ex 
%\textheight=22cm


%\textwidth 15cm
%\oddsidemargin -1cm
%\evensidemargin -1cm

%\headheight=7pt \topmargin=4pt \textheight=604pt 
%\textwidth=432pt
%\oddsidemargin=18pt \evensidemargin=18pt 
%\flushbottom
\usepackage[margin=1in]{geometry}

\parskip=\medskipamount
%\def\baselinestretch{1.2}       % magnification for line spacing
%\def\baselinestretch{1.1}
\def\baselinestretch{1.06}       % magnification for line spacing
%\lineskip=0pt
\lineskip=1.25pt




% \oddsidemargin=0.1in
% \evensidemargin=0.1in
% \marginparwidth=0pt
% \marginparsep=0pt
% \marginparpush=0pt
% \topmargin=0pt
% \headheight=0pt
% \headsep=0pt


\flushbottom





% space above equation (either)
\abovedisplayskip=1em plus.3em minus.5em
% " below
\belowdisplayskip=1em plus.3em minus.5em
% " above when no overlap
\abovedisplayshortskip=.5em plus.2em minus.4em
% " below
\belowdisplayshortskip=.5em plus.2em minus.4em

%%% no headings
\pagestyle{headings}



% Only sections appear in table of contents.
\setcounter{tocdepth}{1}
% Don't force the bottoms of the pages to be at the same spot:
%\raggedbottom
% Allow worse line breaks while this work is in progress.
\tolerance=3000
% We'll get fewer ``underfull hbox'' messages with this set.
\hbadness=4000
% We'll get fewer ``overfull hbox'' messages with this set.
\hfuzz=1pt





